Intrapapillary Capillary Loop Classification in Magnification Endoscopy: Open Dataset and Baseline Methodology

Purpose. Early squamous cell neoplasia (ESCN) in the oesophagus is a highly treatable condition. Lesions confined to the mucosal layer can be curatively treated endoscopically. We build a computer-assisted detection (CADe) system that can classify still images or video frames as normal or abnormal with high diagnostic accuracy. Methods. We present a new benchmark dataset containing 68K binary labeled frames extracted from 114 patient videos whose imaged areas have been resected and correlated to histopathology. Our novel convolutional network (CNN) architecture solves the binary classification task and explains what features of the input domain drive the decision-making process of the network. Results. The proposed method achieved an average accuracy of 91.7 % compared to the 94.7 % achieved by a group of 12 senior clinicians. Our novel network architecture produces deeply supervised activation heatmaps that suggest the network is looking at intrapapillary capillary loop (IPCL) patterns when predicting abnormality. Conclusion. We believe that this dataset and baseline method may serve as a reference for future benchmarks on both video frame classification and explainability in the context of ESCN detection. A future work path of high clinical relevance is the extension of the classification to ESCN types.

==> conclusion.tex <==
%\section{Conclusion}
%\label{sec:conclusion}
%
%Motivated by the need to explain the classification predictions obtained in the context of ESCN, and the limited applicability of standard class activation maps to adapt to this clinical context, we propose a new approach to obtain class activation maps at multiple resolutions embedded into the network architecture. The network generates the class activation maps as part of the inference pipeline. This allows us to visualize relevant input features at different spatial resolutions, allowing for comparison with clinical markers. We evaluate our approach on a magnification endoscopy IPCL dataset that we also make public.
